Wireless Link Scheduling with State-Augmented Graph Neural Networks

We consider the problem of optimal link scheduling in large-scale wireless ad hoc networks. We specifically aim for the maximum long-term average performance, subject to a minimum transmission requirement for each link to ensure fairness. With a graph structure utilized to represent the conflicts of links, we formulate a constrained optimization problem to learn the scheduling policy, which is parameterized with a graph neural network (GNN). To address the challenge of long-term performance, we use the state-augmentation technique. In particular, by augmenting the Lagrangian dual variables as dynamic inputs to the scheduling policy, the GNN can be trained to gradually adapt the scheduling decisions to achieve the minimum transmission requirements. We verify the efficacy of our proposed policy through numerical simulations and compare its performance with several baselines in various network settings.

==> figures/interferencegraph.tex <==
% !TEX root = ../root.tex

\tikzstyle{empty node} = [ circle, 
                           draw = black,
                           text = black, 
                           minimum size = 0.65*\unit]
                           
\tikzstyle{empty node small} = [ circle, 
                           draw = black,
                           text = black, 
                           minimum size = 0.2*\unit]

\tikzstyle{blue node} = [ empty node, 
                         fill = blue!50,
                         draw = blue!50,
                         text = white]

\tikzstyle{red node} = [ empty node, 
                         fill = red!50,
                         draw = red!50,
                         text = white]

\tikzstyle{gray node} = [ empty node, 
                         fill = black!50,
                         draw = black!50,
                         text = white]
                         
\tikzstyle{blue node small} = [ empty node small, 
                         fill = blue!50,
                         draw = blue!50,
                         text = white]
                         
\tikzstyle{gray node small} = [ empty node small, 
                         fill = black!50,
                         draw = black!50,
                         text = white]

\tikzstyle{blue node small next} = [ empty node small, 
                         fill = blue!40,
                         draw = blue!40,
                         text = white]

\tikzstyle{red node small} = [ empty node small, 
                         fill = red!50,
                         draw = red!50,
                         text = white]

\tikzstyle{gray node small next} = [ empty node small, 
                         fill = black!40,
                         draw = black!40,
                         text = white]

\tikzstyle{edge} = [shorten >=0pt, shorten <=0pt]


\def \myfactor {1.00}
\def \unit     {\myfactor cm}

\def \radius   {2.5}


{\fontsize{7}{7}\selectfont\begin{tikzpicture}[scale = 1.2*\myfactor]

 % Nodes in the left pentagon 
  \node                             [blue node small] [label=180:$b$] at (-18,0) (b) {}; % Defines center of pentagon
  \path (b) ++ ( 60:\radius/2+0.2) node [blue node small] (c)   {}; % ++ ( 0.5,  0.5) node {$x_1$}; %;
  \path (b) ++ ( 120:\radius/2+0.2) node [blue node small] [label=$a$] (a)   {}; %  ++ ( 0.6,  0.4) node {$x_2$}; %;
  \path (b) ++ (0: \radius/2+0.2) node [blue node small] [label=0:$c$](e)   {}; %  ++ (-0.6,  0.4) node {$x_3$}; %;
  \path (b) ++ (315:\radius/2+0.2) node [blue node small] (f)   {}; %  ++ (-0.5,  0.5) node {$x_4$}; %;
  
  \path (c) ++ ( 0:\radius/2+0.2 ) node [blue node small] (d)   {};
  
  % \path (3c) ++ (  320 :\radius+0.5 ) node [blue node small next] (k2c)   {$k_2$};


%   % Edges connecting left pentagon  
\draw[line width = 1.5pt] [shorten >=0pt, color = red!50] (a) --node [fill=white,inner sep=2pt]{1} (b);
\draw[line width = 1.5pt] [shorten >=0pt, color = red!50] (b) --node[fill=white,inner sep=2pt]{2} (c);
\draw[line width = 1.5pt] [shorten >=0pt, color = red!50] (c) --node[fill=white,inner sep=2pt]{3} (d);
\draw[line width = 1.5pt] [shorten >=0pt, color = red!50] (c) --node[fill=white,inner sep=2pt]{4} (e);
\draw[line width = 1.5pt] [shorten >=0pt, color = red!50] (b) --node[fill=white,inner sep=2pt]{5} (e);
\draw[line width = 1.5pt] [shorten >=0pt, color = red!50] (b) --node[fill=white,inner sep=2pt]{6} (f);

% \path[-stealth] (1c)  edge [edge] node {} (ic);
%   \path[-stealth] (2c)  edge [edge] node {}  (ic);
%   \path[-stealth] (3c)  edge [edge] node {}  (ic);
%   \draw [shorten >=0pt,dashed] (4c) --node{} (ic);
  
% \draw [shorten >=0pt,dashed] (k1c) --node{} (3c);  
% \path[-stealth] (k2c)  edge [edge] node []{}  (3c);

  % Nodes in the left pentagon 
  \node                             [red node small] at (-15,0) (6) {6}; % Defines center of pentagon
  \path (6) ++ (  60:\radius/2) node [red node small] (1)   {1}; % ++ ( 0.5,  0.5) node {$x_1$}; %;
  \path (1) ++ ( 0:\radius/2) node [red node small] (2)   {2}; %  ++ ( 0.6,  0.4) node {$x_2$}; %;
  \path (2) ++ (300:\radius/2) node [red node small] (3)   {3}; %  ++ (-0.6,  0.4) node {$x_3$}; %;
  \path (3) ++ (240:\radius/2) node [red node small] (4)   {4}; %  ++ (-0.5,  0.5) node {$x_4$}; %;
   \path (4) ++ (180:\radius/2) node [red node small] (5)   {5}; 

  % Edges connecting left pentagon  
  \draw [shorten >=0pt] (6) --node []{} (1);
\draw [shorten >=0pt] (1) --node[]{} (2);
\draw [shorten >=0pt] (2) --node[]{} (3);
\draw [shorten >=0pt] (3) --node[]{} (4);
\draw [shorten >=0pt] (4) --node[]{} (5);
\draw [shorten >=0pt] (5) --node[]{} (6);
\draw [shorten >=0pt] (1) --node[]{} (5);
\draw [shorten >=0pt] (2) --node[]{} (6);
\draw [shorten >=0pt] (2) --node[]{} (5);
\draw [shorten >=0pt] (4) --node[]{} (2);
% \draw [shorten >=0pt] (5) --node[fill=white,inner sep=1pt]{} (6);

  % Nodes in the left pentagon 
%   \node                             [red node small]   at (-7,0)(ib)  {i}; % Defines center of pentagon
%   \path (ib) ++ (  30:\radius/2) node [blue node small] (1b)   {$j_1$}; % ++ ( 0.5,  0.5) node {$x_1$}; %;
%   \path (ib) ++ ( 140:\radius/2+0.5/2 ) node [blue node small] (2b)   {$j_2$}; %  ++ ( 0.6,  0.4) node {$x_2$}; %;
%   \path (ib) ++ (250: \radius/2 -0.5/2) node [blue node small] (3b)   {$j_3$}; %  ++ (-0.6,  0.4) node {$x_3$}; %;
%   \path (ib) ++ (315:\radius/2) node [gray node small] (4b)   {$j_4$}; %  ++ (-0.5,  0.5) node {$x_4$}; %;
  
%   \path (3b) ++ ( 210:\radius ) node [gray node small next] (k1b)   {$k_1$};
  
%   \path (3b) ++ (  320 :\radius+0.5 ) node [blue node small next] (k2b)   {$k_2$};


% %   % Edges connecting left pentagon  
% \path[-stealth] (1b)  edge [edge] node {} (ib);
%   \path[-stealth] (2b)  edge [edge] node {}  (ib);
%   \path[-stealth] (3b)  edge [edge] node {}  (ib);
%   \draw [shorten >=0pt,dashed] (4b) --node{} (ib);
  
%   \path[-stealth] (k1b)  edge [edge] node [fill=white,inner sep=1pt]{$h_{j_3k_1}(t-1)x_{k_1}(t-2)$} (3b);
%   \path[-stealth] (k2b)  edge [edge] node [fill=white,inner sep=1pt]{$h_{j_3 k_2}(t-1)x_{k_2}(t-2)$}  (3b);

%   % Edges connecting right pentagon  
%   \path[stealth-stealth] (6)  edge [edge] node {}  (7);
%   \path[stealth-stealth] (6)  edge [edge] node {}  (8);
%   \path[stealth-stealth] (6)  edge [edge] node {}  (9);
%   \path[stealth-stealth] (6)  edge [edge] node {} (10);
%   \path[stealth-stealth] (7)  edge [edge] node {}  (8);
%   \path[stealth-stealth] (7)  edge [edge] node {}  (9);
%   \path[stealth-stealth] (7)  edge [edge] node {} (10);
%   \path[stealth-stealth] (8)  edge [edge] node {}  (9);
%   \path[stealth-stealth] (8)  edge [edge] node {} (10);
%   \path[stealth-stealth] (9)  edge [edge] node {} (10);

%   % Edges connecting across pentagons (AP Interference). From left to right
%   \path[black!40, -stealth] (1)  edge [edge] node {}  (6);
%   \path[black!40, -stealth] (1)  edge [edge] node {}  (7);
%   \path[black!40, -stealth] (1)  edge [edge] node {}  (8);
%   \path[black!40, -stealth] (1)  edge [edge] node {}  (9);
%   \path[black!40, -stealth] (1)  edge [edge] node {}  (10);


%   % Edges connecting across pentagons (AP Interference). From right to left
%   \path[black!40, -stealth] (6)  edge [edge] node {}  (1);
%   \path[black!40, -stealth] (6)  edge [edge] node {}  (2);
%   \path[black!40, -stealth] (6)  edge [edge] node {}  (3);
%   \path[black!40, -stealth] (6)  edge [edge] node {}  (4);
%   \path[black!40, -stealth] (6)  edge [edge] node {}  (5);



 

%   % Edges connecting right pentagon  
%   \path[stealth-stealth] (6)  edge [edge] node {}  (7);
%   \path[stealth-stealth] (6)  edge [edge] node {}  (8);
%   \path[stealth-stealth] (6)  edge [edge] node {}  (9);
%   \path[stealth-stealth] (6)  edge [edge] node {} (10);
%   \path[stealth-stealth] (7)  edge [edge] node {}  (8);
%   \path[stealth-stealth] (7)  edge [edge] node {}  (9);
%   \path[stealth-stealth] (7)  edge [edge] node {} (10);
%   \path[stealth-stealth] (8)  edge [edge] node {}  (9);
%   \path[stealth-stealth] (8)  edge [edge] node {} (10);
%   \path[stealth-stealth] (9)  edge [edge] node {} (10);

%   % Edges connecting across pentagons (AP Interference). From left to right
%   \path[black!40, -stealth] (1)  edge [edge] node {}  (6);
%   \path[black!40, -stealth] (1)  edge [edge] node {}  (7);
%   \path[black!40, -stealth] (1)  edge [edge] node {}  (8);
%   \path[black!40, -stealth] (1)  edge [edge] node {}  (9);
%   \path[black!40, -stealth] (1)  edge [edge] node {}  (10);


%   % Edges connecting across pentagons (AP Interference). From right to left
%   \path[black!40, -stealth] (6)  edge [edge] node {}  (1);
%   \path[black!40, -stealth] (6)  edge [edge] node {}  (2);
%   \path[black!40, -stealth] (6)  edge [edge] node {}  (3);
%   \path[black!40, -stealth] (6)  edge [edge] node {}  (4);
%   \path[black!40, -stealth] (6)  edge [edge] node {}  (5);


\end{tikzpicture}} 



==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> relatedworks.tex <==
Spatial Deep Learning for Wireless Scheduling

-They learn the optimal scheduling using only the locations of the neighboring transmitters/receivers.
-They design a specific neural network architecture that achieves optimal sum rate.
-They consider average rates as performance, but not over time. They do explain long-term average sum rate, however they use the incremental version and search for an optimal within each time slot. They use instantaneous rates.
-They use weighted sum rate. Most part of the paper uses the same weights for all users, however their introduction of different weights is weird (it is not very natural to add them in the type of architecture they defined). In our case, this would be much easier if we added weights to the edges of the graph (or potentially to the nodes, as a graph signal). They define the weights as indicators of user priorities.
-They test on networks of up to 1250 links.
-They require a dataset that we do not (if we hopefully can transfer adequately)
-They have a network that includes a convolution stage to capture interference patterns and a fully connected stage to capture the nonlinear functional mapping of the optimized schedule. This probably has more trainable parameters than us.
-They test transferability and scalability
-They consider FPLinQ
-"The proposed method achieves near optimal network utility"
-----------------------------------------------------------------------------------
GBLinks: GNN-Based Beam Selection and Link Activation for Ultra-Dense D2D
mmWave Networks

-They consider the problem of joint beam selection and beam activation, for transmitter-receiver pairs within multiple-input multiple-output technologies. The purpose is to control interference between communication pairs in ultra-dense mmWave networks by inactivating some pairs. "The fundamental problems are the user scheduling and the beamforming in multi-user multi-input multi-output (MIMO) wireless communication systems."
-The problem is formulated as a combinatorial optimization problem. Then a Lagrangian dual learning framework is used to train a deep learning model based on a GNN as the problem solution (to find schedulings for beams and links).
-They also lack a minimum tx requirement constraint.
-They test on networks with max 40 tx-rx pairs (not large scale)
-They create many data samples to train their model.
-Their performance does not consider averages.
-"Numerical results demonstrate that the proposed method is near-optimal compared with the existing state-of-art methods"

------------------------------------------------------------------------------------
GRLinQ: A Distributed Link Scheduling
Mechanism with Graph Reinforcement Learning

-This work is sort of based on the 'spatial deep learning for wireless networks' paper
-They propose a hybrid model/data-driven link scheduling mechanism to schedule links between transmitter-receiver pairs. They leverage the benefits of graph reinforcement learning.
-No min tx requirement constraint
-Performance is measured as the average weighted sum rate, although weights are set to 1. The average is done over the links, not over time.
-At each iteration, the RL model decides what some of the undetermined vertices should do (transmit or not) and delay the remaining vertices to later iterations.
-They test on networks with up to 500 links.
-does not claim optimal solution

------------------------------------------------------------------------------------
Link Scheduling Using Graph Neural Networks

-Did not fully understand
-They propose both a centralized and a distributed model based on a graph neural network to solve link scheduling. They consider a conflict graph instead of the comm network graph.
-The scheduling is performed in every time step, avoiding the transmission of two neighboring links in the conflict graph.
-They measure their performance by the approximation ratio to the optimal solution, testing transferability of their model and applying it to networks of 100 links.
-No min tx requirement constraint
-Their performance is not averaged. "the optimal scheduling at each temporal slot is transformed to an MWIS problem in the corresponding conflict graph", they do it within each time slot.
-They have a "weigthed" performance in the sense that they maximize a utility function according to its value for each link? 
-They test in graphs with degree up to 50.
-They don't consider constraints as is, except for link interference, but they also don't have them explicitly expressed.
-d can achieve near optimal performance on small to middle-sized networks

------------------------------------------------------------------------------------
A Machine Learning-Based Algorithm for
Joint Scheduling and Power Control
in Wireless Networks

-Did not fully understand, I would not add it to the related works paragraph
-They formulate the problem of a maximization of the weighted sum rate as a joint nonlinear program. 
-They decompose the problem into two, using a master-slave strategy. Each problem is solved recursively to achieve the optimal solution. The master problem is related to scheduling and flow control, while the slave problem is a power control problem. They integrate SVMs and deep belief networks (DBNs) to solve the slave problem, which is nonlinear.
-They consider a static wireless network.
-They consider small networks.

------------------------------------------------------------------------------------
Geometric Machine Learning Over Riemannian Manifolds for Wireless Link Scheduling

-They maximize the summation of the individual information-theoretic rates over a certain bandwidth. However in the figures they show average sum rate, so they perform some average, but it is not over time (I believe it is within each device with other devices).
-They study the underlying non-Euclidean structures of device-to-device wireless networks. Specifically, they represent local graphs using regularized Laplacian matrices.
-They propose geometric machine learning G-ML for the learning of scheduling decisions. They use a SVM-based learning model for supervised learning. Then they also propose a k-means clustering method for wireless link scheduling problems on Riemannian manifolds.
-They use graphs to represent the network. 
-Their main objective is to solve link scheduling needing fewer training layouts than other state of the art methods.
-They test scalability retraining in networks of different sizes.
-They test transferability to networks of the same size but considering different fading scenarios.
-They have no min tx requirement
-good performance but don't claim an optimal solution
------------------------------------------------------------------------------------
Graph Embedding-Based Wireless Link Scheduling With Few Training Samples

-They propose a method based on a graph embedding to solve the wireless link scheduling problem.
-They generate low-dimensional feature vectors for the graph, and the graph embedding process learns the interference pattern among links.
-The performance is measured using weighted instantaneous sum rate but weights are all 1.
-Their objective, aside from solving link scheduling, is to reduce the number of required training network layouts.
-They test scalability up to 500 links retraining, then transferability up to 100 links.
-no min tx requirement considered.
-"Then, a multi-layer classifier can be used to perform scheduling to near optimum based on the embedding results of each node.", they claim to be optimal with respect to state-of-the-art solutions

------------------------------------------------------------------------------------
GCN-GAN: A Non-linear Temporal Link Prediction Model for Weighted Dynamic Networks

This is, as the title suggests and I potentially ignored it, a link prediction solution. This is not scheduling.

-good performance but do not claim optimal solution
------------------------------------------------------------------------------
GFlow: GNN-Based Optimal Flow Scheduling for Multipath Transmission With Link Overlapping

They propose the use of a DRL based GNN to schedule the optimal flow of a network. The work has some similarities to link scheduling, because the network is represented as a graph and their objective is to maximize total throughput while having some constraints (i.e their links should be transmitting below the corresponding rates). I am almost sure that they do not consider these constraints in their solution. As they don't even consider interferences and they actually schedule flow (which is different to scheduling each link separately), I will not consider this paper.

--------------------------------------------------------------------------------
Graph neural network-based scheduling for multi-UAV-enabled communications in D2D networks

They want to predict the optimal positions and power configurations for all transmitters in a multi-UAV D2D network. They formulate their problem as the maximization of the sum of the rates (no time average), with constrains regarding total power allowed for each device and a minimum transmission constraint. They use a GNN to learn to maximize the rates. In order to consider the constraints, they add to their loss function a penalty term, basically alpha*F(.). The function F expresses the constraint violation, see eq 14 in their paper.

They use several training and testing samples. There are no tests for transferability nor scalability, nor is it explained how the penalty coefficient is chosen or whether there are constraint violations.



INITIAL INTRODUCTION PARAGRAPH I WROTE:
In particular, wireless link scheduling is a critical aspect of resource management that has been studied CITAR ACA TODOS. Its importance lies in its effects for interference mitigation and fairness in the allocation of resources. It is also a factor of importance to provide good quality of service to end users. In \cite{spatialdl} a new architecture is defined to learn the optimal scheduling of links in a network using only geographical locations of users, testing its transferability and scalability. The average rates are considered as a measure of performance, while also considering weights to indicate user priority. \cite{grlinq} use a similar problem formulation, setting priority weights to 1, and improve the model by leveraging the benefits of graph reinforcement learning. There is however no guarantee that all in these two solutions that all links are scheduled at some point in time. The work in \cite{GBlinksbeams} considers the problem of joint beam selection and link activation for ultra-dense mmWave networks, with devices within multiple-input multiple-output (MIMO) technologies. The problem is formulated as a combinatorial optimization problem, using a Lagrangian dual learning framework to train a model based on a GNN and get beam and link schedules. The work uses instantaneous throughput as a performance metric, focusing on small-scale networks of maximum 40 transmitter-receiver pairs. There is however no guarantee that all links are scheduled at some point in time. In \cite{linkschedulingusinggnns} centralized and a distributed models based on GNNs are proposed to solve link scheduling. The interference in the communication network is modeled by using a conflict graph on which training is performed. The performance is measured at every time step by the approximation ratio to the optimal solution. They compare their results to corresponding baselines, considering networks of up to 300 links. There is no guarantee that all links are scheduled at some point in time. The work in \cite{g-mlriemannian} also seeks to maximize the summation of transmission rates, averaging over each device's communication links with other devices. They represent the network using a graph and propose a novel geometric machine learning methodology, based on SVM. They also propose a clustering method for scheduling problems on Riemannian manifolds. One of their main contributions is to lower the number of training layouts required for training. Scalability and transferability to different fading scenarios are both tested. There is no guarantee that all links are ever transmitting. The work in \cite{GNNmultiuav} seeks to predict the optimal positions and power configurations for transmitters in a D2D multi-unmanned aerial vehicle (UAV) network. The objective is the maximization of the total network rate, considering constraints regarding total power allowed for each device and minimum transmission requirements. Their model is based on a GNN, using a loss function with a penalty term to consider the defined constraints. There are no simulations regarding transferability, scalability or satisfaction of constraints.
